Interrupted and cascaded permutation invariant training for speech separation

Permutation Invariant Training (PIT) has long been a stepping stone method for training speech separation model in handling the label ambiguity problem. With PIT selecting the minimum cost label assignments dynamically, very few studies considered the separation problem to be optimizing both the model parameters and the label assignments, but focused on searching for good model architecture and parameters. In this paper, we investigate instead for a given model architecture the various flexible label assignment strategies for training the model, rather than directly using PIT. Surprisingly, we discover a significant performance boost compared to PIT is possible if the model is trained with fixed label assignments and a good set of labels is chosen. With fixed label training cascaded between two sections of PIT, we achieved the state-of-the-art performance on WSJ0-2mix without changing the model architecture at all.

==> tas-22-his.tex <==
epoch sdr
1 9.147658137702942
2 11.070284022235871
3 11.432832601547242
4 12.195201228237153
5 12.81182229309082
6 12.370595868873597
7 13.18337411327362
8 12.7123361287117
9 13.714632866287232
10 13.677724668502808
11 13.978364801025391
12 13.879942210388183
13 12.642919289779663
14 12.715219913864136
15 14.171806995773315
16 14.306315460586548
17 14.687219580078125
18 14.70270532836914
19 14.79036985168457
20 15.165551666641235
21 14.348240408515931
22 15.117383238601684
23 15.09723095741272
24 15.285562734222411
25 15.184680716323852
26 15.334566926193236
27 15.545869370269775
28 15.601331795501709
29 15.412321183013916
30 15.69256383304596
31 15.655926503753662
32 15.014796017837524
33 15.337132875823974
34 15.608426820373536
35 15.612975505828857
36 15.8121402885437
37 15.84582260055542
38 15.81158200340271
39 15.830436476898193
40 15.867288455963134
41 15.819127908706665
42 15.913652450180054
43 15.87833593902588
44 15.9007905254364
45 15.886502187919616
46 15.988527870178222
47 15.974020412826539
48 16.00777114868164
49 16.030008673858642
50 16.035843664550782
51 16.058354120635986
52 16.05943215713501
53 16.02926569786072
54 16.055239435958864
55 16.028046285247804
56 16.091496868896485
57 16.076901319503783
58 16.11365294570923
59 16.08136135673523
60 16.08325662536621
61 16.08179116668701
62 16.13852249221802
63 16.118619955825807
64 16.113300252914428
65 16.14668438606262
66 16.13552886543274
67 16.136201361083984
68 16.101165936660767
69 16.131393046951295
70 16.154534429168702
71 16.133990965652465
72 16.11940903816223
73 16.122337368011475
74 16.11233841018677
75 16.13936008720398
76 16.1458049911499
77 16.12571502532959
78 16.138779306793214
79 16.117777850341795
80 16.12749098892212
81 16.14879431819916
82 16.14363479385376
83 16.149661695861816
84 16.13507861442566
85 16.130682759475707
86 16.139424576568604
87 16.134757969284056
88 16.16717650756836
89 16.139035721969606
90 16.153506673812867
91 16.13029024925232
92 16.14490931739807
93 16.131062615966798
94 16.13137947998047
95 16.15069878349304
96 16.14393429374695
97 16.143097369384765
98 16.175124003219604
99 16.143685474014283
100 16.13695016784668

==> tas-49-3.tex <==
epoch sdr
201 16.562312712097167
202 15.796996572494507
203 16.85241570472717
204 16.657060619735717
205 16.331295683288573
206 16.664906206512452
207 17.154830615997316
208 17.085232064437868
209 17.157235482788085
210 17.29606260032654
211 17.046980701446532
212 16.807997762298584
213 17.001012594604493
214 17.424826898956297
215 17.41268524169922
216 17.42262391433716
217 17.48808850326538
218 17.420839344024657
219 17.533087230682373
220 17.602072421264648
221 17.449061725616456
222 17.580671449279784
223 17.645672550201414
224 17.58175480880737
225 17.578868115615844
226 17.586864458465577
227 17.71955317077637
228 17.783497033691408
229 17.792836890411376
230 17.782234268188475
231 17.756482430267333
232 17.760357441711427
233 17.799312197875977
234 17.854829048538207
235 17.892842463684083
236 17.866247774505617
237 17.862631462860108
238 17.91347255859375
239 17.857377976226807
240 17.858917595672608
241 17.901956256484986
242 17.87711225204468
243 17.93522970123291
244 17.905071134185793
245 17.938179891967774
246 17.95769991760254
247 17.910959756469726
248 17.955319547271728
249 17.92803206100464
250 17.934929206848146
251 17.928774142456053
252 17.923305542755127
253 17.94509902687073
254 17.967465009307862
255 17.92368177947998
256 17.93351983680725
257 17.948785786819457
258 17.968061780548094
259 17.958304833221437
260 17.961340179443358
261 17.95529129562378
262 17.987114248657228
263 17.97459342956543
264 17.936424575042725
265 17.96064921798706
266 17.97663016052246
267 17.99265192642212
268 17.963641954040526
269 17.958058905029297
270 17.952258750152588
271 17.970103942871095
272 17.955625134277344
273 17.95594422225952
274 17.962277310180664
275 17.973751781845092
276 17.975522425842286
277 17.955409603881836
278 17.97353151473999
279 17.97200580062866
280 17.97864490966797
281 17.95662272415161
282 17.969133168029785
283 17.968110706329345
284 17.974910066223146
285 17.960535568237304
286 17.97917826156616
287 17.976643454742433
288 17.981755937576295
289 17.98175443344116
290 17.96528300704956
291 17.99444339981079
292 17.90970090789795
293 17.962907391357422
294 17.96422526550293
295 17.974917248535156
296 17.9573172454834
297 17.973724306488037
298 17.961038379287718
299 17.961540477752685
300 17.989298121643067


==> tas-49.tex <==
epoch sdr
101 8.26449831790924
102 10.238906941890717
103 10.740946749401093
104 11.953856891822815
105 12.640519217300415
106 12.901091395950317
107 13.228796638774872
108 13.312000318527222
109 13.914304877853393
110 13.818727672576903
111 14.02370513973236
112 13.955690787506104
113 14.344944005584717
114 14.606431039428712
115 14.597411881256104
116 14.443371575546264
117 15.027334353637695
118 14.968226022529603
119 15.155675913619994
120 15.005139542007447
121 15.316662668609618
122 15.452900126647949
123 15.50110393447876
124 15.565177888011933
125 15.518360918045044
126 15.4770864818573
127 15.666756676101684
128 15.767255683898926
129 15.273432213973999
130 15.997018803024291
131 15.732010585021973
132 15.926936198425294
133 16.011521084594726
134 16.09710173225403
135 16.077760990905762
136 16.06811111831665
137 16.357336277389525
138 16.08469803314209
139 15.921200998687745
140 16.182531352996826
141 16.737800734329223
142 16.65189802131653
143 16.84385450592041
144 16.839530571365355
145 16.752532677459715
146 16.961412528991698
147 16.930949179840088
148 16.955290911102296
149 16.942802857208253
150 17.185691352844238
151 17.219382498931886
152 17.303875896072388
153 17.257008967971803
154 17.303536011505127
155 17.28178617095947
156 17.43880694065094
157 17.416265557098388
158 17.42586015930176
159 17.426643311309814
160 17.48178083343506
161 17.503947274398804
162 17.52489549255371
163 17.48937763519287
164 17.48474748764038
165 17.531771232223512
166 17.554103267669678
167 17.562429209136962
168 17.538848552703858
169 17.553971614074708
170 17.55958938369751
171 17.55503575973511
172 17.584985903167723
173 17.595683650970457
174 17.621780404663085
175 17.553476207351686
176 17.571684300994875
177 17.592616833877564
178 17.597515087890624
179 17.60830361328125
180 17.580911750030516
181 17.605109782028197
182 17.600251191711425
183 17.617080640411377
184 17.62346604385376
185 17.655647116851807
186 17.625102478027344
187 17.638951489257813
188 17.610465223693847
189 17.609815451049805
190 17.6152002117157
191 17.650775249862672
192 17.647098014068604
193 17.63886372528076
194 17.63245188674927
195 17.64717498245239
196 17.613817903900145
197 17.617561122894287
198 17.614233560943603
199 17.596466284179687
200 17.6196931640625


==> tas-51-his.tex <==
epoch sdr
1 8.953578411245346
2 10.761709038829803
3 11.803319521713258
4 12.04562338924408
5 12.364227000045776
6 13.11130910835266
7 13.385504823493957
8 13.629612168884277
9 13.771622151565552
10 13.93859861755371
11 14.006025354194641
12 14.175931960678101
13 14.443021605682373
14 14.556911861038207
15 14.646566952514648
16 14.82107167224884
17 14.836972646713257
18 14.89179747390747
19 15.03583117980957
20 15.185070741271973
21 15.241568083190918
22 15.379608337402344
23 15.44299743423462
24 15.265860599899291
25 15.508026891708374
26 15.380738849258423
27 15.494924823760986
28 15.724616710662842
29 15.67622209739685
30 15.690080057144165
31 15.664224326324463
32 16.142976528549195
33 16.32847503757477
34 16.288189440917968
35 16.3680209815979
36 16.36990559196472
37 16.469306370544434
38 16.452250872421263
39 16.42748101348877
40 16.56447988052368
41 16.31658998336792
42 16.435306254577636
43 16.477293571090698
44 16.757016263198853
45 16.802698917007447
46 16.8560972032547
47 16.91060308532715
48 16.866841162109374
49 16.85257400932312
50 16.908855741882324
51 17.015209423065187
52 17.0102861038208
53 17.004600296783448
54 17.096380145645142
55 17.054222702407838
56 17.072358380508422
57 17.088596743774414
58 17.149018200302123
59 17.166830096817016
60 17.20163649291992
61 17.172847439956666
62 17.15967830657959
63 17.155247010803222
64 17.208822578048707
65 17.22037942276001
66 17.21325664100647
67 17.2162411567688
68 17.222546933746337
69 17.194050172424316
70 17.21585689430237
71 17.232592517089845
72 17.2221875038147
73 17.219528355789183
74 17.23079713668823
75 17.232348487091066
76 17.253576749801635
77 17.23222064590454
78 17.268701150512694
79 17.255107356643677
80 17.25914704055786
81 17.244881370162965
82 17.25425440750122
83 17.255509440994263
84 17.29001207962036
85 17.285082064056397
86 17.264870167541503
87 17.29216281051636
88 17.2587156124115
89 17.26725233078003
90 17.261275648880005
91 17.273598806762696
92 17.23534762840271
93 17.263470442962646
94 17.30629240722656
95 17.27776202087402
96 17.271489936828612
97 17.300494969940186
98 17.253726881408692
99 17.30125658721924
100 17.257629571914674


==> tas-58-his.tex <==
epoch sdr
1 3.4003090892791747
2 5.94366476726532
3 7.175964495754242
4 8.249743382072449
5 8.7297524435997
6 9.533274624729156
7 9.546727900505067
8 9.731122789049149
9 10.021228569984435
10 10.512789830112457
11 10.249097880744934
12 10.524346806907653
13 10.393649458312987
14 11.04726532382965
15 11.02595700302124
16 11.492131386566163
17 11.653792754793168
18 10.350433478069306
19 11.352017649173737
20 10.604096257972717
21 12.07429786605835
22 12.394796644973756
23 12.358514909505844
24 11.817253566360474
25 12.676837267112733
26 12.225002784347534
27 12.716678060150146
28 12.593933092880249
29 12.602552186203003
30 12.953397117233276
31 10.077911821937562
32 12.75992556438446
33 12.6471426404953
34 13.173256576728821
35 13.244425977897643
36 12.664020849990845
37 12.483236949539185
38 12.268716449356079
39 12.646357996368408
40 13.029924806976318
41 13.016305895996094
42 12.930982954788208
43 13.241509926605225
44 13.05229187889099
45 13.26726942615509
46 13.456768004226685
47 12.884441988754272
48 13.37780124092102
49 13.172262981033326
50 13.734078718948364
51 13.693918090820313
52 13.665848941993714
53 13.78185889854431
54 13.758368191528321
55 13.892984964752197
56 13.700780922698975
57 13.795863666534423
58 13.849880380630493
59 13.970217607498169
60 13.96180163707733
61 13.413332831573486
62 13.847245095825196
63 13.962817725753784
64 13.908048038101196
65 13.957934127807617
66 14.068767028808594
67 13.96205927886963
68 14.171586943435669
69 14.095532424926757
70 14.114917057418824
71 14.149909238433837
72 14.05126996231079
73 14.065205467987061
74 14.086120471191407
75 14.050919592666625
76 14.090867747306824
77 14.074866249847412
78 14.087246641159057
79 14.070502502822876
80 14.080764868545533
81 14.065020492362976
82 14.078669434356689
83 14.105830102920532
84 14.063261608505249
85 14.0890976146698
86 14.123484132766723
87 14.061115800857545
88 14.041750305557251
89 14.12032273979187
90 14.054017573165893
91 14.106425619506837
92 14.105180324172974
93 14.106926747894287
94 14.091587914848327
95 14.119572826004028
96 14.03332695236206
97 14.091221318054199
98 14.040330527877808
99 14.065572220611573
100 14.037055972480774


==> tas-59-his.tex <==
epoch sdr
1 6.460978792762757
2 8.130709652602672
3 9.486188799571991
4 9.45436469552517
5 10.28339992055893
6 9.18216491303444
7 10.869597150611877
8 11.175520261144639
9 11.228786623573303
10 11.943457667160034
11 11.428522028064728
12 11.555761373710633
13 11.635597340011596
14 11.330429915332795
15 12.551085658454895
16 13.14996167831421
17 13.113049044036865
18 12.386096746635436
19 13.041384206581116
20 13.431836576461793
21 13.057341077041626
22 13.65975095062256
23 13.577554057693481
24 13.265492668533325
25 13.55985737247467
26 13.84585556564331
27 13.853844478988648
28 13.766364030838012
29 13.852421662902833
30 13.771781978797913
31 14.049162019157409
32 14.11207571964264
33 14.058969736671449
34 12.17642978439331
35 12.885142776107788
36 12.60250583076477
37 12.841373887252807
38 13.143770239257812
39 12.328786230754853
40 12.748790670204162
41 12.60466745080948
42 13.291945189666748
43 13.624398831558228
44 13.734647371292114
45 13.370126873970031
46 13.64078062210083
47 13.059553279685973
48 14.143540750312805
49 14.154873877334595
50 14.193026788902282
51 14.187800533103943
52 14.330293220901488
53 14.24768331565857
54 14.165437166976929
55 14.417646570587157
56 14.481571728515625
57 14.364717393875122
58 14.504760328674317
59 14.390724018859864
60 14.284164951324463
61 14.512778525161742
62 14.688847032546997
63 14.308934495925904
64 14.59715029144287
65 14.540476432418822
66 14.67457695198059
67 14.689487584304809
68 14.756453573989868
69 14.829563873291015
70 14.926151210021972
71 14.70010971031189
72 14.753323746871947
73 14.893125605773927
74 15.056635461425781
75 14.942393478393555
76 14.990052242279052
77 15.037967680740357
78 15.03388623161316
79 15.087568355941773
80 15.058360824203492
81 15.002279384231567
82 15.124554948806763
83 15.05665658454895
84 14.963231993103028
85 15.140124491119385
86 15.067377709388733
87 15.119509694671631
88 15.072312419509888
89 15.130034426116943
90 15.052746501541138
91 15.130551692962646
92 15.147881702041627
93 15.154364941787719
94 15.138450212097167
95 15.156669869995117
96 15.153882456970214
97 15.154735220336914
98 15.14972081604004
99 15.166696427154541
100 15.112490686416626
101 15.177551487731934

